Correlated Spatiotemporal Evolution of Extreme-Ultraviolet Ribbons and Hard X-rays in a Solar Flare

We analyze the structure and evolution of ribbons from the M7.3 SOL2014-04-18T13 flare using ultraviolet (UV) images from IRIS and SDO/AIA, magnetic data from SDO/HMI, hard X-ray (HXR) images from RHESSI, and light curves from Fermi/GBM, in order to infer properties of coronal magnetic reconnection. As the event progresses, two flare ribbons spread away from the magnetic polarity inversion line. The width of the newly brightened front along the extension of the ribbon is highly intermittent in both space and time, presumably reflecting non-uniformities in the structure and/or dynamics of the flare current sheet. Furthermore, the ribbon width grows most rapidly in regions exhibiting concentrated non-thermal HXR emission, with sharp increases slightly preceding the HXR bursts. The light curve of the ultraviolet emission matches the HXR light curve at photon energies above 25 keV. In other regions the ribbon-width evolution and light curves do not temporally correlate with the HXR emission. This indicates that the production of non-thermal electrons is highly non-uniform within the flare current sheet. Our results suggest a strong connection between the production of non-thermal electrons and the locally enhanced perpendicular extent of flare ribbon fronts, which in turn reflects inhomogeneous structure and/or reconnection dynamics of the current sheet. Despite this variability, the ribbon fronts remain nearly continuous, quasi-one-dimensional features. Thus, although the reconnecting coronal current sheets are highly structured, they remain quasi-two-dimensional and the magnetic energy release occurs systematically, rather than stochastically, through the volume of reconnecting magnetic flux.

==> referee_report.tex <==
Dear Dr. Golub,

We greatly appreciate your effective and efficient handling of our manuscript, as well as the thoughtful response of the referee to our rather lengthy and detailed paper. The presentation has been improved significantly by the revisions requested in the review.

Below, we include each of the referee's comments followed by our response to it. Changes to the manuscript have been made in red typeface to highlight them effectively. We hope that they adequately address the referee's concerns and criticisms.

Best regards,
Stephen J. Naus
Jiong Qiu
C. Richard DeVore
Spiro K. Antiochos
Joel T. Dahlin
James F. Drake
Marc Swisdak

________________________________________________________

The article presents a thorough and well written investigation of the 2D spatial and temporal properties of flare ribbons, well
observed by IRIS, and by using hard X ray data the authors infer properties of the reconnection and particle acceleration
processes and their inherent scales. Better understanding the multi dimensional relationship between corona and chromosphere is an
important step to better understand the flare mechanism and the authors do well to describe this in such detail while making new
insights. I am therefore happy to recommend this article for publication although I have some queries that should be first
addressed or clarified before accepting for publication. 

Thanks. 

Main points: 

1a) In Section 3.4 (line 377) the authors estimate the velocity of the ribbon crossing the chromosphere using their measured
ribbon widths from a single slit jaw image divided by the imaging cadence. I suggest here the authors use the exposure time
instead of the cadence. Since the ribbon width is not calculated here by the difference between two consecutive images the cadence
should not be relevant here in measuring the velocity. Instead the apparent width or 'spreading' of the ribbon is due to its
passage across the image during the time of exposure instead. This factor may account for the authors differences in velocity
compared to those observed by literature.

(a) The ribbon front width is indeed calculated by the difference between the masks of two consecutive images - the mask includes all pixels that are brightened in a given image. A single snapshot of a flare ribbon would include parts of the ribbon that have been brightened earlier and are still cooling. So the newly brightened ribbon fronts have to be derived from the difference between two consecutive images (or masks), and the inferred speed is equivalent to the width divided by the cadence of the images. We have added a sentence in the first paragraph in Section 3.1 to clarify this method. 

(b) The inferred speed of order 40 km/s (10 SJI pixels at the cadence of 28s) is in general agreement with measurements reported in literature. For example, Hinterreiter et al. (2018, Solar Physics, 293, 38) reported the maximum ribbon separation (from PIL) speed in 50 flares, ranging from a few to 60 km/s (Figure 9c in their paper). This is discussed in Section 4 (3rd paragraph) in the manuscript.

1b) In addition, using the full passage of the ribbon leading edge to estimate the inflow speed implies that the projected shape
of this deposition area is essentially a front with zero thickness. Could the authors comment if this is predicted by
models/simulation or if some thickness is expected.

This is a good point. Technically, from the ribbon width alone, we cannot distinguish whether the width of the ribbon front is entirely due to the inflow (mapped in the chromosphere), or due to the thickness of the current sheet undergoing reconnection, or the mixture of the two. It is likely that the width mostly reflects the apparent motion speed, because the inferred speed from the ribbon width (40 km/s) is consistent with the measured speed (up to 30 km/s) from the time-distance brightness diagrams (Figure 9). This is discussed in the third paragraph in Section 4. 

On the other hand, our observations cannot exclude the possibility that the ribbon width evolution might also be associated with the broadening of the current sheet in the corona, as demonstrated in numerical simulations. We have added this discussion with relevant references in the revised manuscript, the 4th paragraph in Section 4. 

2) In the discussion the authors state the variability of brightness or bursty nature of the ribbon is due mostly to the
reconnection process. Yet nowhere do the authors comment on the influence of the non-uniformity of the chromosphere on this
variability. As commonly observed now by IRIS the chromosphere is full of dynamic features of varying density. The response of the
atmosphere to flare heating is also shown by models to be very dependent on initial loop conditions (see recent modelling by both
V. Polito and J. Reep for example). Could the authors add some comment on how much influence would be expected from conditions in
the chromosphere vs those from the magnetic environment.

It is right that the chromosphere is very dynamic and non-uniform, and the structure and pre-flare condition of the chromosphere may affect the brightness of the chromosphere or transition region, produced by energy deposition from the corona. Yet in this study, we track the ribbon brightening by flare heating, which is substantially stronger than, for example, nano-flare heating of the active region or quiescent region (e.g., Polito et al. 2018, ApJ, 856, 278). Therefore we expect that the ribbon brightening signatures are less sensitive to the density variations of the pre-flare chromosphere or corona, and the effect of these variations on the ribbon front width measurements is likely well within the uncertainties in the measurements explored with the changing thresholds in two different passbands sampling different parts of the atmosphere. We have added this discussion in Section 4, third paragraph.

3a) Footnote 3 - Could the authors explain why the SJI 2796 images are not also normalized to DN/s like the 1400?

Since the exposure of SJI 2796 images is constant (8 seconds) at all times, and the ribbon front is detected with a threshold relative to the quiescent brightness, it does not make any difference whether we normalize the image brightness or not. The exposure of the 1400 SJIs varies, so normalization in that passband is necessary. 

3b) Plotting the position of the quiescent region on one of the early context images would be helpful to the reader.

The quiescent region is now indicated in Figure 1c, and described in the caption. Only part of it could be shown because of the choice of the FOV of Figure 1c/d and the subsequent Figure 2 to optimize the presentation of flare ribbon features.

4) Section 3.1 - Line 214 - The authors should mention a little more about why they chose these particular thresholds. Also the
thresholds seem fixed in time. Is the detection number affected by the histogram shifting towards having more brighter pixels as
the flare progresses? Please comment on this.

(a) The particular threshold is chosen based on the time dependent histogram of the pixel brightness in the active region. A fixed threshold is chosen that distinguishes the brightness distribution during the flare from that of the flare-less active region. This method is adopted based on the experience in analyzing many flares observed in TRACE and AIA images in the 1600 passband, where a threshold of 4 times the quiescent brightness well distinguishes the flaring pixels from the plage (e.g. Qiu et al. 2010, ApJ, 725, 319; Kazachenko et al. 2017, ApJ, 845, 49). This is described in Section 3.1, first paragraph. Although the exact values of the threshold are not as well determined for the IRIS SJIs, experiments with varying thresholds guided by the time-dependent histograms provide some conservative measures of the uncertainty with this method, as discussed in Section 3.1, second paragraph. 

(b) If we use larger thresholds as the flare progresses, we will miss pixels of weak brightenings along the ribbons. This is discussed in Section 3.2, and the effect of varying thresholds can be viewed in Figures 6 and 7. Specifically, with the thresholds chosen in this study, for SJI-2796, the total count of ribbon front pixels throughout the flare decreases by 25 percent when using a higher threshold (Figure 6f), and by 12 percent for SJI-1400 (Figure 7f), and the variation in the mean width is trivial (below 1 SJI pixel). We have added this discussion at the end of Section 3.2.

5) In Figure 7 there seems to be a step change in the widths around 47 min from the start. Could the authors discuss if this is
due to the exposure time change? It would be useful if the authors check when the exposure time was cut (assuming the flare
trigger was active) and either plot or mention this in the text somewhere.

At 12:47 UT, the exposure of the SJI-1400 indeed changed from 2.4 to 0.7 second, and subsequently the exposure changed back and forth between 0.4 and 2 seconds (this is described in Footnote 3). Attached plot shows the variations of the SJI-1400 exposure against the measured mean ribbon width. However, it is unlikely that the sharp increase of the ribbon width at 12:47 UT, or variations in the ribbon width in general, be dominated by the change in the exposure, as such variations in the ribbon width are also observed in the measurements with the SJI-2796 (Figure 6e and attached plot), which has a constant exposure time at 8s throughout the flare. This increase of the ribbon width is more likely due to the progress of the flare itself. We have added this discussion in Section 3.2, the second last paragraph.

6) Line 545-553 - Could the authors expand here on how there is little structure in the spreading direction? It is an important
point but at first glance it sounds contradictory to the previous findings of bursty ribbon features. Do they mean that at any
given moment the ribbon has a single profile in brightness taken along the direction of travel. Possibly a reference to Figure 9
would help.

The bursty features only occur at a few places along the ribbon front, but overall the ribbon front appears rather laminar, or quasi-1D. We have rephrased this part. 

7) Line 336 - Could the authors briefly expand on what criteria was used to choose the slit locations?

The slits are chosen so that each of them is roughly perpendicular to the parts of the ribbons it crosses, and crosses a region with enhanced ribbon width, guided by the temporal and spatial distribution of ribbon widths shown in the ribbon width map (Figure 9a). We have expanded this part in Section 3.3, 2nd paragraph. 


Minor points:

Line 215 - Sentence suggests varying exposure time can not be corrected for but the authors have indeed done this. Suggest
rewording.

We have reworded this sentence.

Line 217 - This is a new paragraph so the figure number here (2) would be useful.

Correction has been done.

Line 232 - Suggest 'intersection' instead of 'interception'. Is there a reference for this statement?

References are added, and the word changed.

Line 365 - missing word - the AIA-1600 light curve

Correction has been made. 

Figure 1e/f) There is a zero on the y-axis intersecting the 6 below.

Correction has been made to the figure.

Figure 1e) Are there units for the y-axis?

The units for the 1-8 A SXR light curve by GOES are given in the legend. For clarity of display, the HXR light curves are arbitrarily normalized in this figure. This is clarified in the caption.

Figure 2 - Right hand panels. The scale units imply it is log DN but the numbers don't seem to be the log of the intensity? Again
there are intersecting scale numbers (check the plot routine for the xtickname keyword as you can manually set these).

Corrections to the figure are made.

Figure 3 - The axes seem to be missing on all but one panel of the top sequence.

Axes are added to the top panels.

Figure 4 - Suggest using the same font as the earlier figures. It also looks like the plot in right hand panel is shifted by 10
pixels to the left. The authors should check this.

Corrections are made to the figure.

Figure 5 - Suggest using titles on the figure panels. It's not clear without reading the caption what these figures are. Again the
font should be like the earlier figures.

Done.

Figure 6 - Again the authors could add the N number to the panels to quickly distinguish them

Done.

Footnote 6 - Authors should cite the most the recent work on the point spread function determination. Suggest to check at least
Alissandrakis et al. (2018) and Courrier et al. (2018).

The suggested references are added; on the other hand, Alissandrakis et al. (2018) and Courrier et al. (2018) have determined the PSF for the IRIS SGs, but not for the SJIs. The PSF of the SJI-2796 was recently determined by the IRIS team, and was applied to the data analyzed in this study, which did not suggest significant difference in the ribbon width pattern. This is discussed in Footnote 6.

Line 335 - Time-distance or time vs distance

Done.

Figure 9) Caption: time-distance or time vs distance

Done.

Line 431-342 - Suggest rewording - confusing if the second HXR peak is related or not to the width.

We have revised the statement to simplify it.

Line 445 - Could the authors describe what quasi 2D structure means in this case.

We have corrected this to 1D. %(the reference is to the ribbon front, not the current sheet).

Line 458 - 'This is a signature ...X line'. Is there a reference for this?

We have added a reference to Sturrock (1966).

Line 463 - 'Support this conclusion' The paper is still in prep so I suggest softening to the likes of 'will further investigate /
shed light on'

We have revised this statement to say that the simulated reconnection pattern is laminar, similar to observations. 

Line 465 - Bursty in time and/or space?

We have added "in time and space".

Line 473 - '3 to 4 times the average' Please clarify if this is of IRIS ribbon observations or historical observations. The IRIS PSF will also give a lower limit to the minimum observable width.

The average refers to the IRIS observations in this study; this is clarified in the revised text. 

Line 520 - Where does the scale 10 Mm come from?

We have replaced "an outflow scale" with "a flare-loop height".

Line 560 - 'observations' and '/em' missing latex command?

Corrected.


